Lisan: Yemeni, Iraqi, Libyan, and Sudanese Arabic Dialect Copora with Morphological Annotations

This article presents morphologically-annotated Yemeni, Sudanese, Iraqi, and Libyan Arabic dialects Lisan corpora. Lisan features around 1.2 million tokens. We collected the content of the corpora from several social media platforms. The Yemeni corpus (~ 1.05M tokens) was collected automatically from Twitter. The corpora of the other three dialects (~ 50K tokens each) came manually from Facebook and YouTube posts and comments. Thirty five (35) annotators who are native speakers of the target dialects carried out the annotations. The annotators segemented all words in the four corpora into prefixes, stems and suffixes and labeled each with different morphological features such as part of speech, lemma, and a gloss in English. An Arabic Dialect Annotation Toolkit ADAT was developped for the purpose of the annation. The annotators were trained on a set of guidelines and on how to use ADAT. We developed ADAT to assist the annotators and to ensure compatibility with SAMA and Curras tagsets. The tool is open source, and the four corpora are also available online.

==> eval.tex <==
We evaluated the quality of our corpora in the following manner. 

\begin{itemize} 
\item To ensure overlap in annotations, we also assigned overlapping annotation tasks such that 
more than 5\% of all contexts are by design annotated by more than one annotator. 

\item We ensured that the collected texts belong to the dialect by asking the annotators
to assign a dialect flag to the text. The annotators also provided a dialect lemma when
the MSA lemma differed from the dialect. 

\item \adat's annotation methodology allows token based annotation across texts. 
The annotator selects a token $t$ in the context of one text document $d$. 
The annotator then views other occurrences $t_1,t_2,\ldots,t_n$ of $t$ in other contexts
$d_1,d_2,\ldots,d_n$. 
She also views available annotations for these occurrences without linking the displayed 
annotations to their contexts. 
The annotations either come from MSA morphological analyzers of $t$, or 
from other annotators who have annotated other occurrences of $t$. 

\begin{itemize} 
\item She has the ability to select one of the existing annotations or some of its 
feature annotations as annotations for $t$. 
This speeds up the annotation process and also provides a better 
opportunity for annotation overlap and review. 
\item She selects contexts $D_s \subseteq \{d_1, d_2, \ldots, d_n\}$ with occurrences of $T_s$
that match the semantics of $t$ in $d$. 
This assigns the annotation of $t$ to its occurrences in $D_s$. 
This again improves opportunities for overlap and review. 
\end{itemize} 

\item When an annotator is in doubt of the annotations, they can request review from another 
annotator using the referral functionality. 

\end{itemize} 

\subsection{Quantitative Evaluation}

Given the overlap in the annotations, we performed feature and dialect based inter-annotation
agreement evaluations of the corpora. 
We used the Kappa-Cohen~\cite{j:kappa:McHugh2015} metric as implemented in the Scientific Kit 
Learn (scikit-learn) Python libraries~\cite{w-scikit-learn} to compute the inter-annotation agreement where the number 
of unique categories was below 10,000. 
We used our own implementation when it surpassed 10,000 as the scikit-learn
implementation crashed for 
higher number of categories such as in the Lemma and Stem features. 
We provide the code that reads the corpora, computes the overlap and the inter-annotation scores 
as open source with our corpora as well. 

Tables~\ref{tab:yemen_iaa}, \ref{tab:libya_iaa}, ~\ref{tab:sudan_iaa}, 
and~\ref{tab:iraq_iaa}
show the inter-annotation agreement scores, the number of unique categories, 
the total number of overlaps for annotated features of the 
Yemeni, Libyan, Sudanese and Iraqi corpora, respectively. 

\input{iaa_tables}

\subsection{Qualitative Evaluation}
Although our quantitative analysis results illustrate high agreement between our annotators, there were some disagreements. We broadly classify the reasons of the most frequent mistakes and disagreements into the following groups...


==> iaa_tables.tex <==


\begin{table} 
\begin{tabular}{c|c|c|c|c}  \hline 
        &  Yemeni & Iraqi & Sudanese & Libyan \\ \hline
Overlap & 143,768 & 7,795 &  9,715   & 11,389 \\ 
Stem    &         &       &          &        \\ 
POS     &         &       &          &        \\ 
Lemma   &         &       &          &        \\ 
Prefix  &  733    & 140   &  116     &  184   \\ 
P-POS   &  2,120  & 319   &  496     &  446   \\ 
Suffix  &  1,767  &  299  &  181     &  291   \\
S-POS   &  3,024  & 653   &  861     &  905   \\
Gloss   &         &       &          &        \\
D-Lemma &         &       &          &        \\ 
\end{tabular} 
\caption{Overlap summary across dialects}
\label{tab:overlap} 
\end{table}


\begin{table*}[hb]
    \centering
    
    \resizebox{.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c} \hline 
&\multicolumn{3}{c|}{Strict agreement rules}&&\multicolumn{3}{c|}{Reasonable agreement rules}&&&&\\ \hline
Feature&IAA&Unique&Agree&&IAA&Unique&Agree&&Overlap&NonEmpty&Total\\ \hline
pos&0.726415843&611&225414&&0.999807885&507&280574&&280580&280579&280580\\ \hline
lemma&0.612087189&32807&165604&&0.989986694&24615&267842&&285632&270551&285632\\ \hline
lemma dialect&0.088352951&10&48041&&1&9&108498&&285900&108498&285900\\ \hline
gloss&0.354839332&95318&96021&&0.993658423&70736&268883&&285597&270599&285597\\ \hline
prefix&0.272575563&3528&45972&&0.999393985&2934&151353&&285895&151429&285895\\ \hline
suffix&0.423842786&4997&48324&&0.999633265&3927&106524&&285898&106559&285898\\ \hline
stem&0.660804403&33108&178716&&0.969416271&26825&262177&&285632&270448&285632\\ \hline
voc&0.658720085&93602&178138&&0.991106595&69699&268024&&285637&270429&285637\\ \hline
pos cat&0.711204645&61&74859&&1&58&95699&&283933&95699&283933\\ \hline
gender&0.975461222&2&2050&&1&2&2055&&285900&2055&285900\\ \hline
number&0.997141978&3&2371&&1&3&2374&&285900&2374&285900\\ \hline
voice&1&2&15&&1&2&15&&285900&15&285900\\ \hline
person&1&3&1190&&1&3&1190&&285900&1190&285900\\ \hline
verb aspect&0.858971606&3&14292&&1&3&15471&&285900&15471&285900\\ \hline
pos main&0.800796575&3&84118&&1&3&94243&&285900&94243&285900\\ \hline

    \end{tabular}
}
    \caption{Inter-annotation agreement results for the Yemeni dialect}
    \label{tab:yemen_iaa}
\end{table*}



\begin{table*}[hb]
    \centering
    
    \resizebox{.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c} \hline 
&\multicolumn{3}{c|}{Strict agreement rules}&&\multicolumn{3}{c|}{Reasonable agreement rules}&&&&\\ \hline
Feature&IAA&Unique&Agree&&IAA&Unique&Agree&&Overlap&NonEmpty&Total\\ \hline
pos&0.803896121&131&10138&&0.99988156&107&11803&&11803&11803&11803\\ \hline
lemma&0.571508594&6296&6589&&0.986097399&4613&11361&&11908&11518&11908\\ \hline
lemma dialect&0.398085262&7&4206&&1&6&7196&&11913&7196&11913\\ \hline
gloss&0.331780912&10547&3888&&0.987919723&6889&11439&&11905&11511&11905\\ \hline
prefix&0.198796459&649&1422&&1&497&6269&&11912&6269&11912\\ \hline
suffix&0.406769901&994&2212&&1&739&5004&&11912&5004&11912\\ \hline
stem&0.747401534&5708&8610&&0.969151421&4723&11162&&11908&11517&11908\\ \hline
voc&0.712167317&9290&8205&&0.991661609&7206&11423&&11908&11518&11908\\ \hline
pos cat&0.835664932&40&2252&&1&38&2588&&11888&2588&11888\\ \hline
gender&nan&1&15&&nan&1&15&&11913&15&11913\\ \hline
number&1&2&39&&1&2&39&&11913&39&11913\\ \hline
voice&nan&1&1&&nan&1&1&&11913&1&11913\\ \hline
person&1&3&26&&1&3&26&&11913&26&11913\\ \hline
verb aspect&0.948709289&3&466&&1&3&479&&11913&479&11913\\ \hline
pos main&0.918209679&3&2417&&1&3&2542&&11913&2542&11913\\ \hline
    \end{tabular}
}
    \caption{Inter-annotation agreement results for the Sudanese dialect}
    \label{tab:sudan_iaa}
\end{table*}



\begin{table*}[hb]
    \centering
    \resizebox{.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c} \hline 
&\multicolumn{3}{c|}{Strict agreement rules}&&\multicolumn{3}{c|}{Reasonable agreement rules}&&&&\\ \hline
Feature&IAA&Unique&Agree&&IAA&Unique&Agree&&Overlap&NonEmpty&Total\\ \hline \hline
pos&0.774534617&160&13272&&0.999495313&122&15968&&15968&15968&15968\\ \hline
lemma&0.646066246&6091&9797&&0.991734881&4247&15026&&16194&15149&16194\\ \hline
lemma dialect&0.382886555&7&5557&&1&5&9650&&16240&9650&16240\\ \hline
gloss&0.414080123&11291&6270&&0.984850371&7213&14862&&16235&15063&16235\\ \hline
prefix&0.270741226&533&2199&&0.998359682&367&7210&&16239&7219&16239\\ \hline
suffix&0.446462623&888&2394&&0.999786616&613&4992&&16238&4993&16238\\ \hline
stem&0.69755916&5931&10577&&0.961328238&4672&14568&&16195&15151&16195\\ \hline
voc&0.692072941&9877&10444&&0.987322951&7209&14893&&16194&15081&16194\\ \hline
pos cat&0.832123873&48&5356&&1&44&6188&&16202&6188&16202\\ \hline
gender&1&2&110&&1&2&110&&16240&110&16240\\ \hline
number&1&3&148&&1&3&148&&16240&148&16240\\ \hline
voice&1&2&2&&1&2&2&&16240&2&16240\\ \hline
person&1&3&81&&1&3&81&&16240&81&16240\\ \hline
verb aspect&0.839206335&3&597&&1&3&656&&16240&656&16240\\ \hline
pos main&0.899652206&3&5797&&1&3&6151&&16240&6151&16240\\ \hline
    \end{tabular}
}
    \caption{Inter-annotation agreement results for the Iraqi dialect}
    \label{tab:iraq_iaa}
\end{table*}


\begin{table*}[hb]
    \centering
    
    \resizebox{.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c} \hline 
&\multicolumn{3}{c|}{Strict agreement rules}&&\multicolumn{3}{c|}{Reasonable agreement rules}&&&&\\ \hline
Feature&IAA&Unique&Agree&&IAA&Unique&Agree&&Overlap&NonEmpty&Total\\ \hline
pos&0.738213329&192&11379&&0.999699877&165&14037&&14037&14037&14037\\ \hline
lemma&0.548223802&6633&7242&&0.987559006&4822&13034&&14254&13194&14254\\ \hline
lemma dialect&0.340413203&7&5355&&1&6&9613&&14269&9613&14269\\ \hline
gloss&0.287268393&12206&3790&&0.98834552&7985&12935&&14185&13047&14185\\ \hline
prefix&0.190905889&674&1420&&0.999659504&511&6733&&14269&6735&14269\\ \hline
suffix&0.389629109&1013&2160&&0.999597658&714&5196&&14269&5196&14269\\ \hline
stem&0.651013394&6493&8594&&0.956838557&5182&12626&&14254&13194&14254\\ \hline
voc&0.636587963&10865&8405&&0.989988869&8016&13065&&14254&13190&14254\\ \hline
pos cat&0.845356541&43&2638&&1&38&2987&&14211&2987&14211\\ \hline
gender&1&2&42&&1&2&42&&14269&42&14269\\ \hline
number&0.957272727&3&46&&1&3&47&&14269&47&14269\\ \hline
voice&nan&1&2&&nan&1&2&&14269&2&14269\\ \hline
person&1&3&30&&1&3&30&&14269&30&14269\\ \hline
verb aspect&0.912305064&3&532&&1&3&559&&14269&559&14269\\ \hline
pos main&0.923991113&3&2813&&1&3&2944&&14269&2944&14269\\ \hline
    \end{tabular}
}
    \caption{Inter-annotation agreement results for the Libyan dialect}
    \label{tab:libya_iaa}
\end{table*}



